But that's not why: Inference adjustment by interactive prototype revision

Despite significant advances in machine learning, decision-making of artificial agents is still not perfect and often requires post-hoc human interventions. If the prediction of a model relies on unreasonable factors it is desirable to remove their effect. Deep interactive prototype adjustment enables the user to give hints and correct the model's reasoning. In this paper, we demonstrate that prototypical-part models are well suited for this task as their prediction is based on prototypical image patches that can be interpreted semantically by the user. It shows that even correct classifications can rely on unreasonable prototypes that result from confounding variables in a dataset. Hence, we propose simple yet effective interaction schemes for inference adjustment: The user is consulted interactively to identify faulty prototypes. Non-object prototypes can be removed by prototype masking or a custom mode of deselection training. Interactive prototype rejection allows machine learning na\"{i}ve users to adjust the logic of reasoning without compromising the accuracy.

==> fig.tex <==
\begin{figure}[h]
\begin{minipage}[b]{1.0\linewidth}
\centering
\centerline{\includegraphics[width=11cm]{figs/histogram.png}}
\end{minipage}
\begin{minipage}[b]{1.0\linewidth}
\centering
\centerline{\includegraphics[width=11cm]{figs/accuracy.png}}
\centerline{(a) Effects of prototype revision}\medskip
\end{minipage}
\begin{minipage}[b]{1.0\linewidth}
\centering
\centerline{\includegraphics[width=11cm]{figs/before_after_latent_space4.png}}
\centerline{(b) Movement of prototypes upon iterative revision}\medskip
\end{minipage}
\caption{Prototype revision: (a) Non-object prototypes become sensitive to object features upon iterative revision (upper row). The number of non-object prototypes during iterative revision (lower left). The change in accuracy for different schemes before and after fine-tuning of the last layer (lower right). (b) The prototype vectors (magenta) in non-object areas (blue) move towards areas of object patches (red).
}
\label{masking}
\end{figure}
